Exploring the Limits of Deep Image Clustering using Pretrained Models

We present a general methodology that learns to classify images without labels by leveraging pretrained feature extractors. Our approach involves self-distillation training of clustering heads based on the fact that nearest neighbours in the pretrained feature space are likely to share the same label. We propose a novel objective that learns associations between image features by introducing a variant of pointwise mutual information together with instance weighting. We demonstrate that the proposed objective is able to attenuate the effect of false positive pairs while efficiently exploiting the structure in the pretrained feature space. As a result, we improve the clustering accuracy over $k$-means on $17$ different pretrained models by $6.1$\% and $12.2$\% on ImageNet and CIFAR100, respectively. Finally, using self-supervised vision transformers, we achieve a clustering accuracy of $61.6$\% on ImageNet. The code is available at https://github.com/HHU-MMBS/TEMI-official-BMVC2023.

==> figures/main_figure.tex <==
\begin{wrapfigure}{O}{0.5\textwidth}
\begin{center}
\includegraphics[width=0.5\columnwidth]{figures/overview_fig.pdf}
\end{center}
\caption{\textbf{An overview of the proposed self-distillation clustering framework.} The nearest neighbors are mined in the feature space of $g$. EMA refers to the exponential moving average over the parameters.}
\label{fig:diagram}
\end{wrapfigure}



==> tables/1k1k_poster.tex <==
\begin{table}
\begin{center}
\setlength
\tabcolsep{2pt}  
  \begin{tabular}{lcc}
    \toprule
    Method  & Arch.   & ACC (\%)  \\
    \hline
    SeLa  & Resnet50 & 30.5   \\
    SCAN  & Resnet50    & 39.9   \\
    SSCN& Resnet50    & 41.1  \\
    \midrule
     \multicolumn{3}{l}{\textit{Our method}}\\	
    TEMI DINO  & Resnet50    & 45.2  \\
    TEMI DINO & ViT-B/16     & 58.4   \\
    TEMI MSN & ViT-L/16  & \textbf{61.6}   \\
    \bottomrule
  \end{tabular}
  \end{center}
   \caption{\textbf{Clustering accuracy in \% (ACC) for the ImageNet validation set.}}
   \label{tab:in1k}
\end{table} 


    

==> tables/loss_gains_poster.tex <==
\begin{table}

 \begin{center}
  \begin{tabular}{lccc}
    \toprule
    Method  & Heads & CIFAR100 & ImageNet  \\
    \midrule
    \textit{k}-means & - & 57.0 & 52.3  \\
    SCAN* & 50 & 62.6 & 55.6 \\
    \hline
    PMI & 1 & 61.6 & 57.5  \\
    WPMI & 1 & 63.4 & 56.5 \\
    \hline
    PMI & 50 & 63.1 & 57.7  \\
    WMI & 50 & 65.6 & 57.0 \\
    TEMI & 50 & \textbf{67.1} & \textbf{58.4}  \\
    \bottomrule
  \end{tabular}
  \end{center}
    \caption{\textbf{Ablations with DINO ViT-B/16. ACC is reported.}}
    \label{table:losses}
\end{table}
